Large Language Models are Advanced Anonymizers

Recent privacy research on large language models (LLMs) has shown that they achieve near-human-level performance at inferring personal data from online texts. With ever-increasing model capabilities, existing text anonymization methods are currently lacking behind regulatory requirements and adversarial threats. In this work, we take two steps to bridge this gap: First, we present a new setting for evaluating anonymization in the face of adversarial LLM inferences, allowing for a natural measurement of anonymization performance while remedying some of the shortcomings of previous metrics. Then, within this setting, we develop a novel LLM-based adversarial anonymization framework leveraging the strong inferential capabilities of LLMs to inform our anonymization procedure. We conduct a comprehensive experimental evaluation of adversarial anonymization across 13 LLMs on real-world and synthetic online texts, comparing it against multiple baselines and industry-grade anonymizers. Our evaluation shows that adversarial anonymization outperforms current commercial anonymizers both in terms of the resulting utility and privacy. We support our findings with a human study (n=50) highlighting a strong and consistent human preference for LLM-anonymized texts.

==> Makefile <==
# Makefile, allowing to
# - compile
# - test
# - clean
# - run in docker
# For details, see targets defined below
#
# USAGE, for example: make pdf

#####################
# REQUIRED PACKAGES #
#####################

# For instructions on how to set up your system to run all commands here, follow
# https://hub.docker.com/repository/docker/ethsrilab/latex-plus

##############
# PARAMETERS #
##############

# main
OUTPUTDIR := lqa-output
NAME := main

# special
NOAPPENDIX := $(NAME)_no_appendix
FULL := $(NAME)_full
OVERFULL := $(NAME)_overfull
GRAY := $(NAME)_gray
ABSTRACT := $(OUTPUTDIR)/abstract.txt

# submission
SUBMISSIONDIR := submission
ZIP := submission.zip

# log
LATEXMKDIR := $(OUTPUTDIR)/latexmk
LOG := $(OUTPUTDIR)/$(NAME).log
SHORTLOG := $(OUTPUTDIR)/$(NAME)-short.log

LOGFILES := *.aux *.bbl *.log *.bcf  *.blg *.lot *.toc *.swp *.gz *.out *.ttt *.fls *.fdb_latexmk

# scripts

SCRIPTDIR := lqa/scripts

#############
# COMPILING #
#############

LATEXSCRIPT = ./lqa/latex.sh
LATEX := $(LATEXSCRIPT) $(NAME).tex $(LATEXMKDIR)

##########
# OTHERS #
##########

NOAPPENDIXCONFIG := headers/config/noappendix.config
SHOWOVERFULLCONFIG := headers/config/showoverfull.config

########
# PDFS #
########

.DEFAULT_GOAL := pdf-full

.PHONY: pdf-full
pdf-full:
	# cleanminimal required to remove the root .bbl file (latexmk is confused by this)
	make cleanminimal
	@echo "\n> COMPILING pdf..."
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)/$(FULL).pdf
	@cp $(LATEXMKDIR)/$(NAME).bbl $(OUTPUTDIR) || true
	@cp $(LATEXMKDIR)/$(NAME).log $(LOG)

.PHONY: pdf-appendix
pdf-appendix: pdf-full
	python3 $(SCRIPTDIR)/pages.py --action appendix

# generate labels into the appendix
.PHONY: appendix-labels
appendix-labels: pdf-full
	cat lqa/other/appendix-labels-loader-1.tex > appendix-labels-loader.tex
	# On error "cat: lqa-output/latexmk/appendix.aux: No such file or directory" check if \include{appendix} is still in main.tex 
	cat $(LATEXMKDIR)/appendix.aux >> appendix-labels-loader.tex
	cat lqa/other/appendix-labels-loader-2.tex >> appendix-labels-loader.tex

# generate PDF without the appendix, but with correct labels into the appendix
.PHONY: pdf-no-appendix
pdf-no-appendix: appendix-labels
	# force re-build of latexmk due to missing file
	make clean
	touch $(NOAPPENDIXCONFIG)
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)/$(NOAPPENDIX).pdf
	# cleanminimal is not sufficient as latexmk will not rebuild during next iteration
	make clean

.PHONY: pdf-overfull
pdf-overfull:
	@echo "\n> COMPILING OVERFULL pdf..."
	# force re-build of latexmk due to missing file
	make clean
	touch $(SHOWOVERFULLCONFIG)
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)/$(OVERFULL).pdf
	# cleanminimal is not sufficient as latexmk will not rebuild during next iteration
	make clean

.PHONY: pdf-gray
pdf-gray: pdf-full
	@echo "\n> Producing GRAYSCALE version to $(OUTPUTDIR)/$(GRAY).pdf..."
	gs -sOutputFile=$(OUTPUTDIR)/$(GRAY).pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 -qQUIET -dNOPAUSE -dBATCH $(OUTPUTDIR)/$(FULL).pdf

.PHONY: pdf-all
pdf-all: cleanall
	make pdf-appendix
	make pdf-no-appendix
	make pdf-overfull
	make pdf-gray
	make pdf-full

# build full pdf but also create synctex files
.PHONY: pdf-full-sync
pdf-full-sync: LATEX += "-synctex=1"
pdf-full-sync: pdf-full
	@cp $(LATEXMKDIR)/$(NAME).synctex.gz $(OUTPUTDIR)/$(FULL).synctex.gz || true


# produce better log files
.PHONY: log
log: pdf-full
	pplatex -i $(LOG) > $(SHORTLOG)


###############
# CONVENIENCE #
###############

.PHONY: check
check: pdf-full log
	python3 $(SCRIPTDIR)/checks.py

.PHONY: text
text: pdf-full
	pdftotext $(OUTPUTDIR)/$(FULL).pdf -raw $(OUTPUTDIR)/$(FULL).txt
	sed -z -i 's/-\n//g' $(OUTPUTDIR)/$(FULL).txt
	sed -z -i 's/\n/ /g' $(OUTPUTDIR)/$(FULL).txt

.PHONY: all
all:
	make pdf-all
	make check
	make log

#########
# CLEAN #
#########

# make clean: remove temporary files
.PHONY: clean
clean:
	make cleanminimal
	@echo "\n> CLEANING temporary files..."
	rm -r -f $(LATEXMKDIR) || true
	rm -r -f $(OUTPUTDIR)/script-logs/*.log* || true
	cd $(OUTPUTDIR) && rm -f $(LOGFILES) || true

# make cleanall: remove all produced files
.PHONY: cleanall
cleanall:
	make clean
	@echo "\n> CLEANING PDFs..."
	rm -f *.pdf || true
	rm -f $(OUTPUTDIR)/*.pdf || true
	rm -r -f $(SUBMISSIONDIR) || true
	rm -f appendix-labels-loader.tex
	rm -f $(ABSTRACT)

# make cleanminimal: remove only temporary files in root directory
# - this removes the root .bbl file (latexmk is confused by this)
# - this removes temporary config files (required for appendix loader and overfull)
.PHONY: cleanminimal
cleanminimal:
	@echo "\n> CLEANING minimal files..."
	rm -f $(LOGFILES) || true
	rm -f headers/config/*.config

##############
# SUBMISSION #
##############

.PHONY: abstract
abstract:
	python3 $(SCRIPTDIR)/abstract.py

.PHONY: submission-files
submission-files:
	make cleanall
	make abstract
	# pdf-full omitted as pdf-appendix implicitly runs this
	make pdf-appendix
	make pdf-no-appendix

.PHONY: submission
submission: submission-files check
	@echo "\n> PREPARING submission in directory $(SUBMISSIONDIR)..."
	rm -r -f $(SUBMISSIONDIR)
	mkdir $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/*.pdf $(SUBMISSIONDIR)
	cp $(ABSTRACT) $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/*.bbl $(SUBMISSIONDIR)

.PHONY: zip-no-appendix
zip-no-appendix: submission
	@rm -f $(SUBMISSIONDIR)/$(ZIP)
	make pdf-no-appendix # update output, prepare appendix labels
	touch $(NOAPPENDIXCONFIG) # ensure appendix is not included when compiling again
	zip --quiet -r $(SUBMISSIONDIR)/$(ZIP) . -x /.git* /$(OUTPUTDIR)* /$(SUBMISSIONDIR)/*.zip Makefile
	make cleanminimal

.PHONY: zip-full
zip-full: submission
	@rm -f $(SUBMISSIONDIR)/$(ZIP)
	make pdf-full # update output
	# README_publisher.md is wrong in this case
	zip --quiet -r $(SUBMISSIONDIR)/$(ZIP) . -x /.git* /$(OUTPUTDIR)* /$(SUBMISSIONDIR)/*.zip Makefile README_publisher.md


#########
# ARXIV #
#########

.PHONY: arxiv-files
arxiv-files:
	make clean
	# clean up outdated directories
	rm -rf arxiv ._arXiv

	# create clean directory
	arxiv_latex_cleaner .
	# rename directory
	mv ._arXiv arxiv

	# copy bbl file
	make pdf-full
	cp $(OUTPUTDIR)/*.bbl ./arxiv

	# cleanup
	rm -f arxiv/Makefile arxiv/README.md arxiv/README_publisher.md

.PHONY: arxiv-check
arxiv-check: pdf-full arxiv-files
	# create pdf
	cd arxiv && latexmk -pdf -interaction=nonstopmode $(NAME).tex

	# check resulting pdf
	# requires pdfdiff: https://github.com/cascremers/pdfdiff
	echo "Differences between two PDFs:"
	pdfdiff --diffviewer diff $(OUTPUTDIR)/$(FULL).pdf ./arxiv/$(NAME).pdf

.PHONY: arxiv
arxiv: arxiv-files
	zip -r $(OUTPUTDIR)/arxiv.zip arxiv

##########
# DOCKER #
##########

DOCKER-CMD := ./lqa/docker.sh


PAPERDIR := $$(pwd)
IMAGE := ethsrilab/latex-plus:version-4.0
CONTAINER := latex-plus-container
RUN := $(DOCKER-CMD) run \
		-it \
		--name $(CONTAINER) \
		--workdir="/paper" \
		-v "$(PAPERDIR)":/paper \
		$(IMAGE)

# launch a docker container using the image, which will provide a shell in the container
.PHONY: docker-run
docker-run: clean-container
	$(RUN)

# check for updates and remove the created docker container
.PHONY: clean-container
clean-container:
	$(DOCKER-CMD) pull $(IMAGE)
	$(DOCKER-CMD) rm /$(CONTAINER) 2>/dev/null || true

# all above commands, run in docker
.PHONY: docker-all
docker-all: clean-container
	$(RUN) make all

.PHONY: docker-pdf-full
docker-pdf-full: clean-container
	$(RUN) make pdf-full

.PHONY: docker-pdf-full-sync
docker-pdf-full-sync: clean-container
	$(RUN) make pdf-full-sync

.PHONY: docker-pdf-appendix
docker-pdf-appendix: clean-container
	$(RUN) make pdf-appendix

.PHONY: docker-pdf-no-appendix
docker-pdf-no-appendix: clean-container
	$(RUN) make pdf-no-appendix

.PHONY: docker-pdf-overfull
docker-pdf-overfull: clean-container
	$(RUN) make pdf-overfull

.PHONY: docker-pdf-gray
docker-pdf-gray: clean-container
	$(RUN) make pdf-gray

.PHONY: docker-pdf-all
docker-pdf-all: clean-container
	$(RUN) make pdf-all

.PHONY: docker-submission
docker-submission: clean-container
	$(RUN) make submission

.PHONY: docker-check
docker-check: clean-container
	$(RUN) make check

.PHONY: docker-text
docker-text: clean-container
	$(RUN) make text

.PHONY: docker-zip
docker-zip: clean-container
	$(RUN) make zip

.PHONY: docker-zip-no-appendix
docker-zip-no-appendix: clean-container
	$(RUN) make zip-no-appendix

.PHONY: docker-abstract
docker-abstract: clean-container
	$(RUN) make abstract

.PHONY: docker-arxiv
docker-arxiv: clean-container
	$(RUN) make arxiv

.PHONY: docker-arxiv-check
docker-arxiv-check: clean-container
	$(RUN) make arxiv-check


==> figures/plots/base/all/all/utility_comb_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_comb & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-3.5-AA 1 & 0.892853 & 483 & 772 & 1.886010 & 0.892853 & 0.625648 & GPT-3.5-AA \\
GPT-3.5-AA 2 & 0.852655 & 457 & 772 & 1.658031 & 0.852655 & 0.591969 & GPT-3.5-AA \\
GPT-3.5-AA 3 & 0.839473 & 437 & 772 & 1.542746 & 0.839473 & 0.566062 & GPT-3.5-AA \\
GPT-3.5-AA 4 & 0.824887 & 433 & 772 & 1.488342 & 0.824887 & 0.560881 & GPT-3.5-AA \\
GPT-3.5-AA 5 & 0.810595 & 402 & 772 & 1.344560 & 0.810595 & 0.520725 & GPT-3.5-AA \\
GPT-3.5-Base 1 & 0.912471 & 486 & 772 & 1.908031 & 0.912471 & 0.629534 & GPT-3.5-Base \\
GPT-3.5-Base 2 & 0.894632 & 464 & 772 & 1.713731 & 0.894632 & 0.601036 & GPT-3.5-Base \\
GPT-3.5-Base 3 & 0.881637 & 453 & 772 & 1.637306 & 0.881637 & 0.586788 & GPT-3.5-Base \\
GPT-3.5-Base 4 & 0.873832 & 440 & 772 & 1.569948 & 0.873832 & 0.569948 & GPT-3.5-Base \\
GPT-3.5-Base 5 & 0.868668 & 446 & 772 & 1.571244 & 0.868668 & 0.577720 & GPT-3.5-Base \\
GPT-4-AA 1 & 0.916799 & 461 & 772 & 1.536269 & 0.916799 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.867054 & 382 & 772 & 1.055699 & 0.867054 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.833367 & 350 & 772 & 0.879534 & 0.833367 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.802680 & 329 & 772 & 0.734456 & 0.802680 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.776827 & 321 & 772 & 0.713731 & 0.776827 & 0.415803 & GPT-4-AA \\
GPT-4-Base 1 & 0.926826 & 463 & 772 & 1.634715 & 0.926826 & 0.599741 & GPT-4-Base \\
GPT-4-Base 2 & 0.893151 & 416 & 772 & 1.326425 & 0.893151 & 0.538860 & GPT-4-Base \\
GPT-4-Base 3 & 0.882119 & 411 & 772 & 1.237047 & 0.882119 & 0.532383 & GPT-4-Base \\
GPT-4-Base 4 & 0.868531 & 396 & 772 & 1.145078 & 0.868531 & 0.512953 & GPT-4-Base \\
GPT-4-Base 5 & 0.861736 & 385 & 772 & 1.062176 & 0.861736 & 0.498705 & GPT-4-Base \\
Yi-34B-AA 1 & 0.943188 & 510 & 772 & 2.169689 & 0.943188 & 0.660622 & Yi-34B-AA \\
Yi-34B-AA 2 & 0.925563 & 498 & 772 & 2.056995 & 0.925563 & 0.645078 & Yi-34B-AA \\
Yi-34B-AA 3 & 0.920316 & 493 & 772 & 2.028497 & 0.920316 & 0.638601 & Yi-34B-AA \\
Yi-34B-AA 4 & 0.912324 & 481 & 772 & 1.936528 & 0.912324 & 0.623057 & Yi-34B-AA \\
Yi-34B-AA 5 & 0.907959 & 469 & 772 & 1.873057 & 0.907959 & 0.607513 & Yi-34B-AA \\
Yi-34B-Base 1 & 0.951223 & 528 & 772 & 2.283679 & 0.951223 & 0.683938 & Yi-34B-Base \\
Yi-34B-Base 2 & 0.939418 & 510 & 772 & 2.121762 & 0.939418 & 0.660622 & Yi-34B-Base \\
Yi-34B-Base 3 & 0.935793 & 512 & 772 & 2.128238 & 0.935793 & 0.663212 & Yi-34B-Base \\
Yi-34B-Base 4 & 0.932087 & 503 & 772 & 2.081606 & 0.932087 & 0.651554 & Yi-34B-Base \\
Yi-34B-Base 5 & 0.930402 & 498 & 772 & 2.047927 & 0.930402 & 0.645078 & Yi-34B-Base \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/llama/utility_bleu_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_bleu & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-4-AA 1 & 0.571418 & 461 & 772 & 1.536269 & 0.571418 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.448580 & 382 & 772 & 1.055699 & 0.448580 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.360845 & 350 & 772 & 0.879534 & 0.360845 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.300869 & 329 & 772 & 0.734456 & 0.300869 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.250951 & 321 & 772 & 0.713731 & 0.250951 & 0.415803 & GPT-4-AA \\
Llama3.1-70B 1 & 0.802032 & 477 & 772 & 1.721503 & 0.802032 & 0.617876 & Llama3.1-70B \\
Llama3.1-70B 2 & 0.664682 & 416 & 772 & 1.291451 & 0.664682 & 0.538860 & Llama3.1-70B \\
Llama3.1-70B 3 & 0.563929 & 376 & 772 & 1.049223 & 0.563929 & 0.487047 & Llama3.1-70B \\
Llama3.1-70B 4 & 0.491467 & 358 & 772 & 0.922280 & 0.491467 & 0.463731 & Llama3.1-70B \\
Llama3.1-70B 5 & 0.433846 & 344 & 772 & 0.851036 & 0.433846 & 0.445596 & Llama3.1-70B \\
Llama3.1-8B 1 & 0.768631 & 494 & 772 & 1.898964 & 0.768631 & 0.639896 & Llama3.1-8B \\
Llama3.1-8B 2 & 0.656841 & 443 & 772 & 1.564767 & 0.656841 & 0.573834 & Llama3.1-8B \\
Llama3.1-8B 3 & 0.579386 & 405 & 772 & 1.369171 & 0.579386 & 0.524611 & Llama3.1-8B \\
Llama3.1-8B 4 & 0.529990 & 393 & 772 & 1.243523 & 0.529990 & 0.509067 & Llama3.1-8B \\
Llama3.1-8B 5 & 0.491894 & 384 & 772 & 1.165803 & 0.491894 & 0.497409 & Llama3.1-8B \\
Mistral-7B 1 & 0.441348 & 514 & 772 & 2.027202 & 0.441348 & 0.665803 & Mistral-7B \\
Mistral-7B 2 & 0.357852 & 461 & 772 & 1.669689 & 0.357852 & 0.597150 & Mistral-7B \\
Mistral-7B 3 & 0.326862 & 440 & 772 & 1.522021 & 0.326862 & 0.569948 & Mistral-7B \\
Mistral-7B 4 & 0.314559 & 427 & 772 & 1.471503 & 0.314559 & 0.553109 & Mistral-7B \\
Mistral-7B 5 & 0.300966 & 428 & 772 & 1.427461 & 0.300966 & 0.554404 & Mistral-7B \\
Mixtral-8x22B 1 & 0.628953 & 492 & 772 & 1.856218 & 0.628953 & 0.637306 & Mixtral-8x22B \\
Mixtral-8x22B 2 & 0.491341 & 423 & 772 & 1.468912 & 0.491341 & 0.547927 & Mixtral-8x22B \\
Mixtral-8x22B 3 & 0.409979 & 393 & 772 & 1.240933 & 0.409979 & 0.509067 & Mixtral-8x22B \\
Mixtral-8x22B 4 & 0.356469 & 383 & 772 & 1.136010 & 0.356469 & 0.496114 & Mixtral-8x22B \\
Mixtral-8x22B 5 & 0.325582 & 373 & 772 & 1.080311 & 0.325582 & 0.483161 & Mixtral-8x22B \\
Mixtral-8x7B 1 & 0.459654 & 515 & 772 & 2.072539 & 0.459654 & 0.667098 & Mixtral-8x7B \\
Mixtral-8x7B 2 & 0.353858 & 476 & 772 & 1.731865 & 0.353858 & 0.616580 & Mixtral-8x7B \\
Mixtral-8x7B 3 & 0.308679 & 447 & 772 & 1.528497 & 0.308679 & 0.579016 & Mixtral-8x7B \\
Mixtral-8x7B 4 & 0.273714 & 430 & 772 & 1.423575 & 0.273714 & 0.556995 & Mixtral-8x7B \\
Mixtral-8x7B 5 & 0.252351 & 419 & 772 & 1.322539 & 0.252351 & 0.542746 & Mixtral-8x7B \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/llama/utility_comb_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_comb & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-4-AA 1 & 0.916799 & 461 & 772 & 1.536269 & 0.916799 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.867054 & 382 & 772 & 1.055699 & 0.867054 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.833367 & 350 & 772 & 0.879534 & 0.833367 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.802680 & 329 & 772 & 0.734456 & 0.802680 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.776827 & 321 & 772 & 0.713731 & 0.776827 & 0.415803 & GPT-4-AA \\
Llama3.1-70B 1 & 0.921780 & 477 & 772 & 1.721503 & 0.921780 & 0.617876 & Llama3.1-70B \\
Llama3.1-70B 2 & 0.870402 & 416 & 772 & 1.291451 & 0.870402 & 0.538860 & Llama3.1-70B \\
Llama3.1-70B 3 & 0.838617 & 376 & 772 & 1.049223 & 0.838617 & 0.487047 & Llama3.1-70B \\
Llama3.1-70B 4 & 0.814069 & 358 & 772 & 0.922280 & 0.814069 & 0.463731 & Llama3.1-70B \\
Llama3.1-70B 5 & 0.793861 & 344 & 772 & 0.851036 & 0.793861 & 0.445596 & Llama3.1-70B \\
Llama3.1-8B 1 & 0.885473 & 494 & 772 & 1.898964 & 0.885473 & 0.639896 & Llama3.1-8B \\
Llama3.1-8B 2 & 0.838674 & 443 & 772 & 1.564767 & 0.838674 & 0.573834 & Llama3.1-8B \\
Llama3.1-8B 3 & 0.809151 & 405 & 772 & 1.369171 & 0.809151 & 0.524611 & Llama3.1-8B \\
Llama3.1-8B 4 & 0.785921 & 393 & 772 & 1.243523 & 0.785921 & 0.509067 & Llama3.1-8B \\
Llama3.1-8B 5 & 0.773792 & 384 & 772 & 1.165803 & 0.773792 & 0.497409 & Llama3.1-8B \\
Mistral-7B 1 & 0.895629 & 514 & 772 & 2.027202 & 0.895629 & 0.665803 & Mistral-7B \\
Mistral-7B 2 & 0.858563 & 461 & 772 & 1.669689 & 0.858563 & 0.597150 & Mistral-7B \\
Mistral-7B 3 & 0.832099 & 440 & 772 & 1.522021 & 0.832099 & 0.569948 & Mistral-7B \\
Mistral-7B 4 & 0.822023 & 427 & 772 & 1.471503 & 0.822023 & 0.553109 & Mistral-7B \\
Mistral-7B 5 & 0.808264 & 428 & 772 & 1.427461 & 0.808264 & 0.554404 & Mistral-7B \\
Mixtral-8x22B 1 & 0.913048 & 492 & 772 & 1.856218 & 0.913048 & 0.637306 & Mixtral-8x22B \\
Mixtral-8x22B 2 & 0.878811 & 423 & 772 & 1.468912 & 0.878811 & 0.547927 & Mixtral-8x22B \\
Mixtral-8x22B 3 & 0.851807 & 393 & 772 & 1.240933 & 0.851807 & 0.509067 & Mixtral-8x22B \\
Mixtral-8x22B 4 & 0.828300 & 383 & 772 & 1.136010 & 0.828300 & 0.496114 & Mixtral-8x22B \\
Mixtral-8x22B 5 & 0.810454 & 373 & 772 & 1.080311 & 0.810454 & 0.483161 & Mixtral-8x22B \\
Mixtral-8x7B 1 & 0.910840 & 515 & 772 & 2.072539 & 0.910840 & 0.667098 & Mixtral-8x7B \\
Mixtral-8x7B 2 & 0.871982 & 476 & 772 & 1.731865 & 0.871982 & 0.616580 & Mixtral-8x7B \\
Mixtral-8x7B 3 & 0.837979 & 447 & 772 & 1.528497 & 0.837979 & 0.579016 & Mixtral-8x7B \\
Mixtral-8x7B 4 & 0.807366 & 430 & 772 & 1.423575 & 0.807366 & 0.556995 & Mixtral-8x7B \\
Mixtral-8x7B 5 & 0.778981 & 419 & 772 & 1.322539 & 0.778981 & 0.542746 & Mixtral-8x7B \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/llama/utility_model_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_model & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-4-AA 1 & 0.927267 & 461 & 772 & 1.536269 & 0.927267 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.887694 & 382 & 772 & 1.055699 & 0.887694 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.866062 & 350 & 772 & 0.879534 & 0.866062 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.844041 & 329 & 772 & 0.734456 & 0.844041 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.826166 & 321 & 772 & 0.713731 & 0.826166 & 0.415803 & GPT-4-AA \\
Llama3.1-70B 1 & 0.929016 & 477 & 772 & 1.721503 & 0.929016 & 0.617876 & Llama3.1-70B \\
Llama3.1-70B 2 & 0.885816 & 416 & 772 & 1.291451 & 0.885816 & 0.538860 & Llama3.1-70B \\
Llama3.1-70B 3 & 0.864832 & 376 & 772 & 1.049223 & 0.864832 & 0.487047 & Llama3.1-70B \\
Llama3.1-70B 4 & 0.847984 & 358 & 772 & 0.922280 & 0.847984 & 0.463731 & Llama3.1-70B \\
Llama3.1-70B 5 & 0.835816 & 344 & 772 & 0.851036 & 0.835816 & 0.445596 & Llama3.1-70B \\
Llama3.1-8B 1 & 0.883225 & 494 & 772 & 1.898964 & 0.883225 & 0.639896 & Llama3.1-8B \\
Llama3.1-8B 2 & 0.841775 & 443 & 772 & 1.564767 & 0.841775 & 0.573834 & Llama3.1-8B \\
Llama3.1-8B 3 & 0.817746 & 405 & 772 & 1.369171 & 0.817746 & 0.524611 & Llama3.1-8B \\
Llama3.1-8B 4 & 0.799935 & 393 & 772 & 1.243523 & 0.799935 & 0.509067 & Llama3.1-8B \\
Llama3.1-8B 5 & 0.791386 & 384 & 772 & 1.165803 & 0.791386 & 0.497409 & Llama3.1-8B \\
Mistral-7B 1 & 0.920596 & 514 & 772 & 2.027202 & 0.920596 & 0.665803 & Mistral-7B \\
Mistral-7B 2 & 0.892746 & 461 & 772 & 1.669689 & 0.892746 & 0.597150 & Mistral-7B \\
Mistral-7B 3 & 0.867422 & 440 & 772 & 1.522021 & 0.867422 & 0.569948 & Mistral-7B \\
Mistral-7B 4 & 0.861334 & 427 & 772 & 1.471503 & 0.861334 & 0.553109 & Mistral-7B \\
Mistral-7B 5 & 0.847215 & 428 & 772 & 1.427461 & 0.847215 & 0.554404 & Mistral-7B \\
Mixtral-8x22B 1 & 0.918135 & 492 & 772 & 1.856218 & 0.918135 & 0.637306 & Mixtral-8x22B \\
Mixtral-8x22B 2 & 0.892034 & 423 & 772 & 1.468912 & 0.892034 & 0.547927 & Mixtral-8x22B \\
Mixtral-8x22B 3 & 0.872345 & 393 & 772 & 1.240933 & 0.872345 & 0.509067 & Mixtral-8x22B \\
Mixtral-8x22B 4 & 0.853627 & 383 & 772 & 1.136010 & 0.853627 & 0.496114 & Mixtral-8x22B \\
Mixtral-8x22B 5 & 0.840544 & 373 & 772 & 1.080311 & 0.840544 & 0.483161 & Mixtral-8x22B \\
Mixtral-8x7B 1 & 0.923640 & 515 & 772 & 2.072539 & 0.923640 & 0.667098 & Mixtral-8x7B \\
Mixtral-8x7B 2 & 0.891127 & 476 & 772 & 1.731865 & 0.891127 & 0.616580 & Mixtral-8x7B \\
Mixtral-8x7B 3 & 0.860816 & 447 & 772 & 1.528497 & 0.860816 & 0.579016 & Mixtral-8x7B \\
Mixtral-8x7B 4 & 0.834521 & 430 & 772 & 1.423575 & 0.834521 & 0.556995 & Mixtral-8x7B \\
Mixtral-8x7B 5 & 0.805829 & 419 & 772 & 1.322539 & 0.805829 & 0.542746 & Mixtral-8x7B \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/llama/utility_rouge_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_rouge & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-4-AA 1 & 0.895863 & 461 & 772 & 1.536269 & 0.895863 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.825774 & 382 & 772 & 1.055699 & 0.825774 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.767977 & 350 & 772 & 0.879534 & 0.767977 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.719958 & 329 & 772 & 0.734456 & 0.719958 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.678148 & 321 & 772 & 0.713731 & 0.678148 & 0.415803 & GPT-4-AA \\
Llama3.1-70B 1 & 0.907309 & 477 & 772 & 1.721503 & 0.907309 & 0.617876 & Llama3.1-70B \\
Llama3.1-70B 2 & 0.839575 & 416 & 772 & 1.291451 & 0.839575 & 0.538860 & Llama3.1-70B \\
Llama3.1-70B 3 & 0.786188 & 376 & 772 & 1.049223 & 0.786188 & 0.487047 & Llama3.1-70B \\
Llama3.1-70B 4 & 0.743886 & 358 & 772 & 0.922280 & 0.743886 & 0.463731 & Llama3.1-70B \\
Llama3.1-70B 5 & 0.709952 & 344 & 772 & 0.851036 & 0.709952 & 0.445596 & Llama3.1-70B \\
Llama3.1-8B 1 & 0.889968 & 494 & 772 & 1.898964 & 0.889968 & 0.639896 & Llama3.1-8B \\
Llama3.1-8B 2 & 0.832473 & 443 & 772 & 1.564767 & 0.832473 & 0.573834 & Llama3.1-8B \\
Llama3.1-8B 3 & 0.791960 & 405 & 772 & 1.369171 & 0.791960 & 0.524611 & Llama3.1-8B \\
Llama3.1-8B 4 & 0.757894 & 393 & 772 & 1.243523 & 0.757894 & 0.509067 & Llama3.1-8B \\
Llama3.1-8B 5 & 0.738605 & 384 & 772 & 1.165803 & 0.738605 & 0.497409 & Llama3.1-8B \\
Mistral-7B 1 & 0.845696 & 514 & 772 & 2.027202 & 0.845696 & 0.665803 & Mistral-7B \\
Mistral-7B 2 & 0.790197 & 461 & 772 & 1.669689 & 0.790197 & 0.597150 & Mistral-7B \\
Mistral-7B 3 & 0.761452 & 440 & 772 & 1.522021 & 0.761452 & 0.569948 & Mistral-7B \\
Mistral-7B 4 & 0.743401 & 427 & 772 & 1.471503 & 0.743401 & 0.553109 & Mistral-7B \\
Mistral-7B 5 & 0.730362 & 428 & 772 & 1.427461 & 0.730362 & 0.554404 & Mistral-7B \\
Mixtral-8x22B 1 & 0.902873 & 492 & 772 & 1.856218 & 0.902873 & 0.637306 & Mixtral-8x22B \\
Mixtral-8x22B 2 & 0.852365 & 423 & 772 & 1.468912 & 0.852365 & 0.547927 & Mixtral-8x22B \\
Mixtral-8x22B 3 & 0.810731 & 393 & 772 & 1.240933 & 0.810731 & 0.509067 & Mixtral-8x22B \\
Mixtral-8x22B 4 & 0.777647 & 383 & 772 & 1.136010 & 0.777647 & 0.496114 & Mixtral-8x22B \\
Mixtral-8x22B 5 & 0.750273 & 373 & 772 & 1.080311 & 0.750273 & 0.483161 & Mixtral-8x22B \\
Mixtral-8x7B 1 & 0.885241 & 515 & 772 & 2.072539 & 0.885241 & 0.667098 & Mixtral-8x7B \\
Mixtral-8x7B 2 & 0.833692 & 476 & 772 & 1.731865 & 0.833692 & 0.616580 & Mixtral-8x7B \\
Mixtral-8x7B 3 & 0.792305 & 447 & 772 & 1.528497 & 0.792305 & 0.579016 & Mixtral-8x7B \\
Mixtral-8x7B 4 & 0.753056 & 430 & 772 & 1.423575 & 0.753056 & 0.556995 & Mixtral-8x7B \\
Mixtral-8x7B 5 & 0.725285 & 419 & 772 & 1.322539 & 0.725285 & 0.542746 & Mixtral-8x7B \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/qwen/utility_bleu_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_bleu & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-4-AA 1 & 0.571418 & 461 & 772 & 1.536269 & 0.571418 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.448580 & 382 & 772 & 1.055699 & 0.448580 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.360845 & 350 & 772 & 0.879534 & 0.360845 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.300869 & 329 & 772 & 0.734456 & 0.300869 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.250951 & 321 & 772 & 0.713731 & 0.250951 & 0.415803 & GPT-4-AA \\
Qwen1.5-14B-AA 1 & 0.535953 & 555 & 772 & 2.380829 & 0.535953 & 0.718912 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 2 & 0.359598 & 486 & 772 & 1.889896 & 0.359598 & 0.629534 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 3 & 0.281209 & 460 & 772 & 1.720207 & 0.281209 & 0.595855 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 4 & 0.240534 & 440 & 772 & 1.601036 & 0.240534 & 0.569948 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 5 & 0.200487 & 423 & 772 & 1.474093 & 0.200487 & 0.547927 & Qwen1.5-14B-AA \\
Qwen1.5-32B-AA 1 & 0.416351 & 502 & 772 & 1.979275 & 0.416351 & 0.650259 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 2 & 0.286135 & 461 & 772 & 1.594560 & 0.286135 & 0.597150 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 3 & 0.233654 & 412 & 772 & 1.353627 & 0.233654 & 0.533679 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 4 & 0.190524 & 422 & 772 & 1.318653 & 0.190524 & 0.546632 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 5 & 0.169639 & 407 & 772 & 1.238342 & 0.169639 & 0.527202 & Qwen1.5-32B-AA \\
Qwen1.5-4B-AA 1 & 0.661092 & 612 & 772 & 2.946891 & 0.661092 & 0.792746 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 2 & 0.582905 & 591 & 772 & 2.791451 & 0.582905 & 0.765544 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 3 & 0.550195 & 575 & 772 & 2.721503 & 0.550195 & 0.744819 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 4 & 0.537391 & 566 & 772 & 2.639896 & 0.537391 & 0.733161 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 5 & 0.526348 & 561 & 772 & 2.613990 & 0.526348 & 0.726684 & Qwen1.5-4B-AA \\
Qwen2-72B-AA 1 & 0.751630 & 467 & 772 & 1.682642 & 0.751630 & 0.604922 & Qwen2-72B-AA \\
Qwen2-72B-AA 2 & 0.635115 & 421 & 772 & 1.309585 & 0.635115 & 0.545337 & Qwen2-72B-AA \\
Qwen2-72B-AA 3 & 0.553573 & 382 & 772 & 1.150259 & 0.553573 & 0.494819 & Qwen2-72B-AA \\
Qwen2-72B-AA 4 & 0.497636 & 375 & 772 & 1.029793 & 0.497636 & 0.485751 & Qwen2-72B-AA \\
Qwen2-72B-AA 5 & 0.460676 & 368 & 772 & 0.985751 & 0.460676 & 0.476684 & Qwen2-72B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/qwen/utility_comb_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_comb & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-4-AA 1 & 0.916799 & 461 & 772 & 1.536269 & 0.916799 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.867054 & 382 & 772 & 1.055699 & 0.867054 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.833367 & 350 & 772 & 0.879534 & 0.833367 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.802680 & 329 & 772 & 0.734456 & 0.802680 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.776827 & 321 & 772 & 0.713731 & 0.776827 & 0.415803 & GPT-4-AA \\
Qwen1.5-14B-AA 1 & 0.867046 & 555 & 772 & 2.380829 & 0.867046 & 0.718912 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 2 & 0.810513 & 486 & 772 & 1.889896 & 0.810513 & 0.629534 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 3 & 0.770208 & 460 & 772 & 1.720207 & 0.770208 & 0.595855 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 4 & 0.742100 & 440 & 772 & 1.601036 & 0.742100 & 0.569948 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 5 & 0.724436 & 423 & 772 & 1.474093 & 0.724436 & 0.547927 & Qwen1.5-14B-AA \\
Qwen1.5-32B-AA 1 & 0.893633 & 502 & 772 & 1.979275 & 0.893633 & 0.650259 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 2 & 0.848652 & 461 & 772 & 1.594560 & 0.848652 & 0.597150 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 3 & 0.821760 & 412 & 772 & 1.353627 & 0.821760 & 0.533679 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 4 & 0.794495 & 422 & 772 & 1.318653 & 0.794495 & 0.546632 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 5 & 0.779674 & 407 & 772 & 1.238342 & 0.779674 & 0.527202 & Qwen1.5-32B-AA \\
Qwen1.5-4B-AA 1 & 0.863957 & 612 & 772 & 2.946891 & 0.863957 & 0.792746 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 2 & 0.824466 & 591 & 772 & 2.791451 & 0.824466 & 0.765544 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 3 & 0.800092 & 575 & 772 & 2.721503 & 0.800092 & 0.744819 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 4 & 0.789516 & 566 & 772 & 2.639896 & 0.789516 & 0.733161 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 5 & 0.781697 & 561 & 772 & 2.613990 & 0.781697 & 0.726684 & Qwen1.5-4B-AA \\
Qwen2-72B-AA 1 & 0.896933 & 467 & 772 & 1.682642 & 0.896933 & 0.604922 & Qwen2-72B-AA \\
Qwen2-72B-AA 2 & 0.855687 & 421 & 772 & 1.309585 & 0.855687 & 0.545337 & Qwen2-72B-AA \\
Qwen2-72B-AA 3 & 0.825060 & 382 & 772 & 1.150259 & 0.825060 & 0.494819 & Qwen2-72B-AA \\
Qwen2-72B-AA 4 & 0.799981 & 375 & 772 & 1.029793 & 0.799981 & 0.485751 & Qwen2-72B-AA \\
Qwen2-72B-AA 5 & 0.783598 & 368 & 772 & 0.985751 & 0.783598 & 0.476684 & Qwen2-72B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/qwen/utility_model_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_model & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-4-AA 1 & 0.927267 & 461 & 772 & 1.536269 & 0.927267 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.887694 & 382 & 772 & 1.055699 & 0.887694 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.866062 & 350 & 772 & 0.879534 & 0.866062 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.844041 & 329 & 772 & 0.734456 & 0.844041 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.826166 & 321 & 772 & 0.713731 & 0.826166 & 0.415803 & GPT-4-AA \\
Qwen1.5-14B-AA 1 & 0.897021 & 555 & 772 & 2.380829 & 0.897021 & 0.718912 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 2 & 0.861464 & 486 & 772 & 1.889896 & 0.861464 & 0.629534 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 3 & 0.829883 & 460 & 772 & 1.720207 & 0.829883 & 0.595855 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 4 & 0.807383 & 440 & 772 & 1.601036 & 0.807383 & 0.569948 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 5 & 0.795785 & 423 & 772 & 1.474093 & 0.795785 & 0.547927 & Qwen1.5-14B-AA \\
Qwen1.5-32B-AA 1 & 0.922927 & 502 & 772 & 1.979275 & 0.922927 & 0.650259 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 2 & 0.898834 & 461 & 772 & 1.594560 & 0.898834 & 0.597150 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 3 & 0.885104 & 412 & 772 & 1.353627 & 0.885104 & 0.533679 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 4 & 0.865674 & 422 & 772 & 1.318653 & 0.865674 & 0.546632 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 5 & 0.855699 & 407 & 772 & 1.238342 & 0.855699 & 0.527202 & Qwen1.5-32B-AA \\
Qwen1.5-4B-AA 1 & 0.875583 & 612 & 772 & 2.946891 & 0.875583 & 0.792746 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 2 & 0.838536 & 591 & 772 & 2.791451 & 0.838536 & 0.765544 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 3 & 0.813636 & 575 & 772 & 2.721503 & 0.813636 & 0.744819 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 4 & 0.804275 & 566 & 772 & 2.639896 & 0.804275 & 0.733161 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 5 & 0.796956 & 561 & 772 & 2.613990 & 0.796956 & 0.726684 & Qwen1.5-4B-AA \\
Qwen2-72B-AA 1 & 0.902073 & 467 & 772 & 1.682642 & 0.902073 & 0.604922 & Qwen2-72B-AA \\
Qwen2-72B-AA 2 & 0.872215 & 421 & 772 & 1.309585 & 0.872215 & 0.545337 & Qwen2-72B-AA \\
Qwen2-72B-AA 3 & 0.848640 & 382 & 772 & 1.150259 & 0.848640 & 0.494819 & Qwen2-72B-AA \\
Qwen2-72B-AA 4 & 0.827073 & 375 & 772 & 1.029793 & 0.827073 & 0.485751 & Qwen2-72B-AA \\
Qwen2-72B-AA 5 & 0.814249 & 368 & 772 & 0.985751 & 0.814249 & 0.476684 & Qwen2-72B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/qwen/utility_rouge_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_rouge & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-4-AA 1 & 0.895863 & 461 & 772 & 1.536269 & 0.895863 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.825774 & 382 & 772 & 1.055699 & 0.825774 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.767977 & 350 & 772 & 0.879534 & 0.767977 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.719958 & 329 & 772 & 0.734456 & 0.719958 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.678148 & 321 & 772 & 0.713731 & 0.678148 & 0.415803 & GPT-4-AA \\
Qwen1.5-14B-AA 1 & 0.807097 & 555 & 772 & 2.380829 & 0.807097 & 0.718912 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 2 & 0.708610 & 486 & 772 & 1.889896 & 0.708610 & 0.629534 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 3 & 0.647758 & 460 & 772 & 1.720207 & 0.647758 & 0.595855 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 4 & 0.611533 & 440 & 772 & 1.601036 & 0.611533 & 0.569948 & Qwen1.5-14B-AA \\
Qwen1.5-14B-AA 5 & 0.581267 & 423 & 772 & 1.474093 & 0.581267 & 0.547927 & Qwen1.5-14B-AA \\
Qwen1.5-32B-AA 1 & 0.835044 & 502 & 772 & 1.979275 & 0.835044 & 0.650259 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 2 & 0.748288 & 461 & 772 & 1.594560 & 0.748288 & 0.597150 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 3 & 0.695074 & 412 & 772 & 1.353627 & 0.695074 & 0.533679 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 4 & 0.652137 & 422 & 772 & 1.318653 & 0.652137 & 0.546632 & Qwen1.5-32B-AA \\
Qwen1.5-32B-AA 5 & 0.627622 & 407 & 772 & 1.238342 & 0.627622 & 0.527202 & Qwen1.5-32B-AA \\
Qwen1.5-4B-AA 1 & 0.840704 & 612 & 772 & 2.946891 & 0.840704 & 0.792746 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 2 & 0.796324 & 591 & 772 & 2.791451 & 0.796324 & 0.765544 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 3 & 0.771092 & 575 & 772 & 2.721503 & 0.771092 & 0.744819 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 4 & 0.759998 & 566 & 772 & 2.639896 & 0.759998 & 0.733161 & Qwen1.5-4B-AA \\
Qwen1.5-4B-AA 5 & 0.751179 & 561 & 772 & 2.613990 & 0.751179 & 0.726684 & Qwen1.5-4B-AA \\
Qwen2-72B-AA 1 & 0.886652 & 467 & 772 & 1.682642 & 0.886652 & 0.604922 & Qwen2-72B-AA \\
Qwen2-72B-AA 2 & 0.822632 & 421 & 772 & 1.309585 & 0.822632 & 0.545337 & Qwen2-72B-AA \\
Qwen2-72B-AA 3 & 0.777899 & 382 & 772 & 1.150259 & 0.777899 & 0.494819 & Qwen2-72B-AA \\
Qwen2-72B-AA 4 & 0.745797 & 375 & 772 & 1.029793 & 0.745797 & 0.485751 & Qwen2-72B-AA \\
Qwen2-72B-AA 5 & 0.722296 & 368 & 772 & 0.985751 & 0.722296 & 0.476684 & Qwen2-72B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/rest/utility_bleu_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_bleu & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
Dipper 1 & 0.177167 & 629 & 772 & 3.055699 & 0.177167 & 0.814767 & Dipper \\
Dipper 2 & 0.137239 & 605 & 772 & 2.928756 & 0.137239 & 0.783679 & Dipper \\
Dipper 3 & 0.125435 & 615 & 772 & 2.946891 & 0.125435 & 0.796632 & Dipper \\
Dipper 4 & 0.119554 & 606 & 772 & 2.838083 & 0.119554 & 0.784974 & Dipper \\
Dipper 5 & 0.116777 & 608 & 772 & 2.902850 & 0.116777 & 0.787565 & Dipper \\
Dou-SD 1 & 0.303888 & 524 & 772 & 2.168394 & 0.303888 & 0.678756 & Dou-SD \\
GPT-4-AA 1 & 0.571418 & 461 & 772 & 1.536269 & 0.571418 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.448580 & 382 & 772 & 1.055699 & 0.448580 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.360845 & 350 & 772 & 0.879534 & 0.360845 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.300869 & 329 & 772 & 0.734456 & 0.300869 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.250951 & 321 & 772 & 0.713731 & 0.250951 & 0.415803 & GPT-4-AA \\
Gemma2-27B 1 & 0.920988 & 537 & 772 & 2.360104 & 0.920988 & 0.695596 & Gemma2-27B \\
Gemma2-27B 2 & 0.885232 & 499 & 772 & 2.094560 & 0.885232 & 0.646373 & Gemma2-27B \\
Gemma2-27B 3 & 0.860558 & 480 & 772 & 1.976684 & 0.860558 & 0.621762 & Gemma2-27B \\
Gemma2-27B 4 & 0.845076 & 480 & 772 & 1.924870 & 0.845076 & 0.621762 & Gemma2-27B \\
Gemma2-27B 5 & 0.832650 & 477 & 772 & 1.835492 & 0.832650 & 0.617876 & Gemma2-27B \\
Mistral-7B 1 & 0.441348 & 514 & 772 & 2.027202 & 0.441348 & 0.665803 & Mistral-7B \\
Mistral-7B 2 & 0.357852 & 461 & 772 & 1.669689 & 0.357852 & 0.597150 & Mistral-7B \\
Mistral-7B 3 & 0.326862 & 440 & 772 & 1.522021 & 0.326862 & 0.569948 & Mistral-7B \\
Mistral-7B 4 & 0.314559 & 427 & 772 & 1.471503 & 0.314559 & 0.553109 & Mistral-7B \\
Mistral-7B 5 & 0.300966 & 428 & 772 & 1.427461 & 0.300966 & 0.554404 & Mistral-7B \\
Yi-34B-AA 1 & 0.534505 & 510 & 772 & 2.169689 & 0.534505 & 0.660622 & Yi-34B-AA \\
Yi-34B-AA 2 & 0.491969 & 498 & 772 & 2.056995 & 0.491969 & 0.645078 & Yi-34B-AA \\
Yi-34B-AA 3 & 0.472283 & 493 & 772 & 2.028497 & 0.472283 & 0.638601 & Yi-34B-AA \\
Yi-34B-AA 4 & 0.456250 & 481 & 772 & 1.936528 & 0.456250 & 0.623057 & Yi-34B-AA \\
Yi-34B-AA 5 & 0.438201 & 469 & 772 & 1.873057 & 0.438201 & 0.607513 & Yi-34B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/rest/utility_comb_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_comb & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
Dipper 1 & 0.879029 & 629 & 772 & 3.055699 & 0.879029 & 0.814767 & Dipper \\
Dipper 2 & 0.847819 & 605 & 772 & 2.928756 & 0.847819 & 0.783679 & Dipper \\
Dipper 3 & 0.838287 & 615 & 772 & 2.946891 & 0.838287 & 0.796632 & Dipper \\
Dipper 4 & 0.829421 & 606 & 772 & 2.838083 & 0.829421 & 0.784974 & Dipper \\
Dipper 5 & 0.833728 & 608 & 772 & 2.902850 & 0.833728 & 0.787565 & Dipper \\
Dou-SD 1 & 0.815928 & 524 & 772 & 2.168394 & 0.815928 & 0.678756 & Dou-SD \\
GPT-4-AA 1 & 0.916799 & 461 & 772 & 1.536269 & 0.916799 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.867054 & 382 & 772 & 1.055699 & 0.867054 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.833367 & 350 & 772 & 0.879534 & 0.833367 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.802680 & 329 & 772 & 0.734456 & 0.802680 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.776827 & 321 & 772 & 0.713731 & 0.776827 & 0.415803 & GPT-4-AA \\
Gemma2-27B 1 & 0.951572 & 537 & 772 & 2.360104 & 0.951572 & 0.695596 & Gemma2-27B \\
Gemma2-27B 2 & 0.931523 & 499 & 772 & 2.094560 & 0.931523 & 0.646373 & Gemma2-27B \\
Gemma2-27B 3 & 0.916964 & 480 & 772 & 1.976684 & 0.916964 & 0.621762 & Gemma2-27B \\
Gemma2-27B 4 & 0.910310 & 480 & 772 & 1.924870 & 0.910310 & 0.621762 & Gemma2-27B \\
Gemma2-27B 5 & 0.903618 & 477 & 772 & 1.835492 & 0.903618 & 0.617876 & Gemma2-27B \\
Mistral-7B 1 & 0.895629 & 514 & 772 & 2.027202 & 0.895629 & 0.665803 & Mistral-7B \\
Mistral-7B 2 & 0.858563 & 461 & 772 & 1.669689 & 0.858563 & 0.597150 & Mistral-7B \\
Mistral-7B 3 & 0.832099 & 440 & 772 & 1.522021 & 0.832099 & 0.569948 & Mistral-7B \\
Mistral-7B 4 & 0.822023 & 427 & 772 & 1.471503 & 0.822023 & 0.553109 & Mistral-7B \\
Mistral-7B 5 & 0.808264 & 428 & 772 & 1.427461 & 0.808264 & 0.554404 & Mistral-7B \\
Yi-34B-AA 1 & 0.943188 & 510 & 772 & 2.169689 & 0.943188 & 0.660622 & Yi-34B-AA \\
Yi-34B-AA 2 & 0.925563 & 498 & 772 & 2.056995 & 0.925563 & 0.645078 & Yi-34B-AA \\
Yi-34B-AA 3 & 0.920316 & 493 & 772 & 2.028497 & 0.920316 & 0.638601 & Yi-34B-AA \\
Yi-34B-AA 4 & 0.912324 & 481 & 772 & 1.936528 & 0.912324 & 0.623057 & Yi-34B-AA \\
Yi-34B-AA 5 & 0.907959 & 469 & 772 & 1.873057 & 0.907959 & 0.607513 & Yi-34B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/rest/utility_model_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_model & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
Dipper 1 & 0.927655 & 629 & 772 & 3.055699 & 0.927655 & 0.814767 & Dipper \\
Dipper 2 & 0.906347 & 605 & 772 & 2.928756 & 0.906347 & 0.783679 & Dipper \\
Dipper 3 & 0.901425 & 615 & 772 & 2.946891 & 0.901425 & 0.796632 & Dipper \\
Dipper 4 & 0.892940 & 606 & 772 & 2.838083 & 0.892940 & 0.784974 & Dipper \\
Dipper 5 & 0.901166 & 608 & 772 & 2.902850 & 0.901166 & 0.787565 & Dipper \\
Dou-SD 1 & 0.848899 & 524 & 772 & 2.168394 & 0.848899 & 0.678756 & Dou-SD \\
GPT-4-AA 1 & 0.927267 & 461 & 772 & 1.536269 & 0.927267 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.887694 & 382 & 772 & 1.055699 & 0.887694 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.866062 & 350 & 772 & 0.879534 & 0.866062 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.844041 & 329 & 772 & 0.734456 & 0.844041 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.826166 & 321 & 772 & 0.713731 & 0.826166 & 0.415803 & GPT-4-AA \\
Gemma2-27B 1 & 0.945984 & 537 & 772 & 2.360104 & 0.945984 & 0.695596 & Gemma2-27B \\
Gemma2-27B 2 & 0.925259 & 499 & 772 & 2.094560 & 0.925259 & 0.646373 & Gemma2-27B \\
Gemma2-27B 3 & 0.909909 & 480 & 772 & 1.976684 & 0.909909 & 0.621762 & Gemma2-27B \\
Gemma2-27B 4 & 0.903821 & 480 & 772 & 1.924870 & 0.903821 & 0.621762 & Gemma2-27B \\
Gemma2-27B 5 & 0.897345 & 477 & 772 & 1.835492 & 0.897345 & 0.617876 & Gemma2-27B \\
Mistral-7B 1 & 0.920596 & 514 & 772 & 2.027202 & 0.920596 & 0.665803 & Mistral-7B \\
Mistral-7B 2 & 0.892746 & 461 & 772 & 1.669689 & 0.892746 & 0.597150 & Mistral-7B \\
Mistral-7B 3 & 0.867422 & 440 & 772 & 1.522021 & 0.867422 & 0.569948 & Mistral-7B \\
Mistral-7B 4 & 0.861334 & 427 & 772 & 1.471503 & 0.861334 & 0.553109 & Mistral-7B \\
Mistral-7B 5 & 0.847215 & 428 & 772 & 1.427461 & 0.847215 & 0.554404 & Mistral-7B \\
Yi-34B-AA 1 & 0.946244 & 510 & 772 & 2.169689 & 0.946244 & 0.660622 & Yi-34B-AA \\
Yi-34B-AA 2 & 0.928756 & 498 & 772 & 2.056995 & 0.928756 & 0.645078 & Yi-34B-AA \\
Yi-34B-AA 3 & 0.925842 & 493 & 772 & 2.028497 & 0.925842 & 0.638601 & Yi-34B-AA \\
Yi-34B-AA 4 & 0.916256 & 481 & 772 & 1.936528 & 0.916256 & 0.623057 & Yi-34B-AA \\
Yi-34B-AA 5 & 0.913083 & 469 & 772 & 1.873057 & 0.913083 & 0.607513 & Yi-34B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/score_ablation/rest/utility_rouge_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_rouge & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
Dipper 1 & 0.781775 & 629 & 772 & 3.055699 & 0.781775 & 0.814767 & Dipper \\
Dipper 2 & 0.730764 & 605 & 772 & 2.928756 & 0.730764 & 0.783679 & Dipper \\
Dipper 3 & 0.712011 & 615 & 772 & 2.946891 & 0.712011 & 0.796632 & Dipper \\
Dipper 4 & 0.702382 & 606 & 772 & 2.838083 & 0.702382 & 0.784974 & Dipper \\
Dipper 5 & 0.698852 & 608 & 772 & 2.902850 & 0.698852 & 0.787565 & Dipper \\
Dou-SD 1 & 0.749987 & 524 & 772 & 2.168394 & 0.749987 & 0.678756 & Dou-SD \\
GPT-4-AA 1 & 0.895863 & 461 & 772 & 1.536269 & 0.895863 & 0.597150 & GPT-4-AA \\
GPT-4-AA 2 & 0.825774 & 382 & 772 & 1.055699 & 0.825774 & 0.494819 & GPT-4-AA \\
GPT-4-AA 3 & 0.767977 & 350 & 772 & 0.879534 & 0.767977 & 0.453368 & GPT-4-AA \\
GPT-4-AA 4 & 0.719958 & 329 & 772 & 0.734456 & 0.719958 & 0.426166 & GPT-4-AA \\
GPT-4-AA 5 & 0.678148 & 321 & 772 & 0.713731 & 0.678148 & 0.415803 & GPT-4-AA \\
Gemma2-27B 1 & 0.962746 & 537 & 772 & 2.360104 & 0.962746 & 0.695596 & Gemma2-27B \\
Gemma2-27B 2 & 0.944052 & 499 & 772 & 2.094560 & 0.944052 & 0.646373 & Gemma2-27B \\
Gemma2-27B 3 & 0.931074 & 480 & 772 & 1.976684 & 0.931074 & 0.621762 & Gemma2-27B \\
Gemma2-27B 4 & 0.923287 & 480 & 772 & 1.924870 & 0.923287 & 0.621762 & Gemma2-27B \\
Gemma2-27B 5 & 0.916165 & 477 & 772 & 1.835492 & 0.916165 & 0.617876 & Gemma2-27B \\
Mistral-7B 1 & 0.845696 & 514 & 772 & 2.027202 & 0.845696 & 0.665803 & Mistral-7B \\
Mistral-7B 2 & 0.790197 & 461 & 772 & 1.669689 & 0.790197 & 0.597150 & Mistral-7B \\
Mistral-7B 3 & 0.761452 & 440 & 772 & 1.522021 & 0.761452 & 0.569948 & Mistral-7B \\
Mistral-7B 4 & 0.743401 & 427 & 772 & 1.471503 & 0.743401 & 0.553109 & Mistral-7B \\
Mistral-7B 5 & 0.730362 & 428 & 772 & 1.427461 & 0.730362 & 0.554404 & Mistral-7B \\
Yi-34B-AA 1 & 0.937076 & 510 & 772 & 2.169689 & 0.937076 & 0.660622 & Yi-34B-AA \\
Yi-34B-AA 2 & 0.919175 & 498 & 772 & 2.056995 & 0.919175 & 0.645078 & Yi-34B-AA \\
Yi-34B-AA 3 & 0.909264 & 493 & 772 & 2.028497 & 0.909264 & 0.638601 & Yi-34B-AA \\
Yi-34B-AA 4 & 0.904459 & 481 & 772 & 1.936528 & 0.904459 & 0.623057 & Yi-34B-AA \\
Yi-34B-AA 5 & 0.897711 & 469 & 772 & 1.873057 & 0.897711 & 0.607513 & Yi-34B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/synthetic/all/all/pii_type_=all/correct_full_anon_setting.tex <==
\begin{tabular}{lr}
\toprule
pii_type & first_correct \\
\midrule
AGE & 599 \\
EDU & 977 \\
INC & 727 \\
LOC & 388 \\
OCCP & 324 \\
POBP & 216 \\
REL & 812 \\
SEX & 1021 \\
\bottomrule
\end{tabular}


==> figures/plots/synthetic/all/all/utility_comb_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_comb & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
Dou-SD 1 & 0.827258 & 288 & 525 & 1.847619 & 0.827258 & 0.558422 & Dou-SD \\
Dou-SD 2 & 0.757390 & 261 & 525 & 1.603810 & 0.757390 & 0.506070 & Dou-SD \\
Dou-SD 3 & 0.738550 & 244 & 525 & 1.422857 & 0.738550 & 0.473107 & Dou-SD \\
GPT-3.5-AA 1 & 0.872358 & 227 & 525 & 1.302857 & 0.872358 & 0.440145 & GPT-3.5-AA \\
GPT-3.5-AA 2 & 0.812196 & 199 & 525 & 1.034286 & 0.812196 & 0.385854 & GPT-3.5-AA \\
GPT-3.5-AA 3 & 0.769448 & 176 & 525 & 0.857143 & 0.769448 & 0.341258 & GPT-3.5-AA \\
GPT-4-AA 1 & 0.913275 & 197 & 525 & 1.013333 & 0.913275 & 0.381976 & GPT-4-AA \\
GPT-4-AA 2 & 0.840454 & 162 & 525 & 0.697143 & 0.840454 & 0.314112 & GPT-4-AA \\
GPT-4-AA 3 & 0.803533 & 135 & 525 & 0.520000 & 0.803533 & 0.261760 & GPT-4-AA \\
Llama3.1-70B-AA 1 & 0.928240 & 221 & 525 & 1.201905 & 0.928240 & 0.428511 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 2 & 0.877338 & 164 & 525 & 0.771429 & 0.877338 & 0.317990 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 3 & 0.838736 & 149 & 525 & 0.647619 & 0.838736 & 0.288906 & Llama3.1-70B-AA \\
Llama3.1-8B-AA 1 & 0.924701 & 207 & 454 & 1.409692 & 0.924701 & 0.401366 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 2 & 0.885096 & 173 & 454 & 1.048458 & 0.885096 & 0.335441 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 3 & 0.854769 & 155 & 454 & 0.859031 & 0.854769 & 0.300540 & Llama3.1-8B-AA \\
Mistral-7B-AA 1 & 0.901095 & 250 & 525 & 1.493333 & 0.901095 & 0.484741 & Mistral-7B-AA \\
Mistral-7B-AA 2 & 0.871076 & 235 & 525 & 1.306667 & 0.871076 & 0.455657 & Mistral-7B-AA \\
Mistral-7B-AA 3 & 0.856468 & 230 & 525 & 1.255238 & 0.856468 & 0.445962 & Mistral-7B-AA \\
Yi-34B-AA 1 & 0.924301 & 265 & 525 & 1.615238 & 0.924301 & 0.513826 & Yi-34B-AA \\
Yi-34B-AA 2 & 0.912855 & 247 & 525 & 1.436190 & 0.912855 & 0.478924 & Yi-34B-AA \\
Yi-34B-AA 3 & 0.901958 & 242 & 525 & 1.382857 & 0.901958 & 0.469229 & Yi-34B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/synthetic/all/all/utility_model_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_model & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
Dou-SD 1 & 0.862952 & 288 & 525 & 1.847619 & 0.862952 & 0.558422 & Dou-SD \\
Dou-SD 2 & 0.803238 & 261 & 525 & 1.603810 & 0.803238 & 0.506070 & Dou-SD \\
Dou-SD 3 & 0.786762 & 244 & 525 & 1.422857 & 0.786762 & 0.473107 & Dou-SD \\
GPT-3.5-AA 1 & 0.892762 & 227 & 525 & 1.302857 & 0.892762 & 0.440145 & GPT-3.5-AA \\
GPT-3.5-AA 2 & 0.855524 & 199 & 525 & 1.034286 & 0.855524 & 0.385854 & GPT-3.5-AA \\
GPT-3.5-AA 3 & 0.813238 & 176 & 525 & 0.857143 & 0.813238 & 0.341258 & GPT-3.5-AA \\
GPT-4-AA 1 & 0.926762 & 197 & 525 & 1.013333 & 0.926762 & 0.381976 & GPT-4-AA \\
GPT-4-AA 2 & 0.877143 & 162 & 525 & 0.697143 & 0.877143 & 0.314112 & GPT-4-AA \\
GPT-4-AA 3 & 0.862952 & 135 & 525 & 0.520000 & 0.862952 & 0.261760 & GPT-4-AA \\
Llama3.1-70B-AA 1 & 0.940667 & 221 & 525 & 1.201905 & 0.940667 & 0.428511 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 2 & 0.909810 & 164 & 525 & 0.771429 & 0.909810 & 0.317990 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 3 & 0.892667 & 149 & 525 & 0.647619 & 0.892667 & 0.288906 & Llama3.1-70B-AA \\
Llama3.1-8B-AA 1 & 0.934692 & 207 & 454 & 1.409692 & 0.934692 & 0.401366 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 2 & 0.907269 & 173 & 454 & 1.048458 & 0.907269 & 0.335441 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 3 & 0.887115 & 155 & 454 & 0.859031 & 0.887115 & 0.300540 & Llama3.1-8B-AA \\
Mistral-7B-AA 1 & 0.927143 & 250 & 525 & 1.493333 & 0.927143 & 0.484741 & Mistral-7B-AA \\
Mistral-7B-AA 2 & 0.914286 & 235 & 525 & 1.306667 & 0.914286 & 0.455657 & Mistral-7B-AA \\
Mistral-7B-AA 3 & 0.904857 & 230 & 525 & 1.255238 & 0.904857 & 0.445962 & Mistral-7B-AA \\
Yi-34B-AA 1 & 0.926857 & 265 & 525 & 1.615238 & 0.926857 & 0.513826 & Yi-34B-AA \\
Yi-34B-AA 2 & 0.921048 & 247 & 525 & 1.436190 & 0.921048 & 0.478924 & Yi-34B-AA \\
Yi-34B-AA 3 & 0.908762 & 242 & 525 & 1.382857 & 0.908762 & 0.469229 & Yi-34B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/synthetic/all/all/utility_rouge_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_rouge & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
Dou-SD 1 & 0.755869 & 288 & 525 & 1.847619 & 0.755869 & 0.558422 & Dou-SD \\
Dou-SD 2 & 0.665693 & 261 & 525 & 1.603810 & 0.665693 & 0.506070 & Dou-SD \\
Dou-SD 3 & 0.642126 & 244 & 525 & 1.422857 & 0.642126 & 0.473107 & Dou-SD \\
GPT-3.5-AA 1 & 0.831550 & 227 & 525 & 1.302857 & 0.831550 & 0.440145 & GPT-3.5-AA \\
GPT-3.5-AA 2 & 0.725541 & 199 & 525 & 1.034286 & 0.725541 & 0.385854 & GPT-3.5-AA \\
GPT-3.5-AA 3 & 0.681867 & 176 & 525 & 0.857143 & 0.681867 & 0.341258 & GPT-3.5-AA \\
GPT-4-AA 1 & 0.886302 & 197 & 525 & 1.013333 & 0.886302 & 0.381976 & GPT-4-AA \\
GPT-4-AA 2 & 0.767078 & 162 & 525 & 0.697143 & 0.767078 & 0.314112 & GPT-4-AA \\
GPT-4-AA 3 & 0.684695 & 135 & 525 & 0.520000 & 0.684695 & 0.261760 & GPT-4-AA \\
Llama3.1-70B-AA 1 & 0.903387 & 221 & 525 & 1.201905 & 0.903387 & 0.428511 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 2 & 0.812396 & 164 & 525 & 0.771429 & 0.812396 & 0.317990 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 3 & 0.730874 & 149 & 525 & 0.647619 & 0.730874 & 0.288906 & Llama3.1-70B-AA \\
Llama3.1-8B-AA 1 & 0.904720 & 207 & 454 & 1.409692 & 0.904720 & 0.401366 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 2 & 0.840751 & 173 & 454 & 1.048458 & 0.840751 & 0.335441 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 3 & 0.790078 & 155 & 454 & 0.859031 & 0.790078 & 0.300540 & Llama3.1-8B-AA \\
Mistral-7B-AA 1 & 0.848999 & 250 & 525 & 1.493333 & 0.848999 & 0.484741 & Mistral-7B-AA \\
Mistral-7B-AA 2 & 0.784658 & 235 & 525 & 1.306667 & 0.784658 & 0.455657 & Mistral-7B-AA \\
Mistral-7B-AA 3 & 0.759689 & 230 & 525 & 1.255238 & 0.759689 & 0.445962 & Mistral-7B-AA \\
Yi-34B-AA 1 & 0.919189 & 265 & 525 & 1.615238 & 0.919189 & 0.513826 & Yi-34B-AA \\
Yi-34B-AA 2 & 0.896469 & 247 & 525 & 1.436190 & 0.896469 & 0.478924 & Yi-34B-AA \\
Yi-34B-AA 3 & 0.888351 & 242 & 525 & 1.382857 & 0.888351 & 0.469229 & Yi-34B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/synthpai/utility_comb_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_comb & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-3.5-AA 1 & 0.934460 & 261 & 477 & 1.817610 & 0.934460 & 0.547170 & GPT-3.5-AA \\
GPT-3.5-AA 2 & 0.913475 & 243 & 477 & 1.637317 & 0.913475 & 0.509434 & GPT-3.5-AA \\
GPT-3.5-AA 3 & 0.894875 & 224 & 477 & 1.457023 & 0.894875 & 0.469602 & GPT-3.5-AA \\
GPT-4-AA 1 & 0.916789 & 182 & 477 & 0.958071 & 0.916789 & 0.381551 & GPT-4-AA \\
GPT-4-AA 2 & 0.866004 & 140 & 477 & 0.624738 & 0.866004 & 0.293501 & GPT-4-AA \\
GPT-4-AA 3 & 0.829308 & 125 & 477 & 0.511530 & 0.829308 & 0.262055 & GPT-4-AA \\
Llama3.1-70B-AA 1 & 0.923048 & 187 & 477 & 1.037736 & 0.923048 & 0.392034 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 2 & 0.887077 & 162 & 477 & 0.756813 & 0.887077 & 0.339623 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 3 & 0.857628 & 149 & 477 & 0.637317 & 0.857628 & 0.312369 & Llama3.1-70B-AA \\
Llama3.1-8B-AA 1 & 0.914579 & 256 & 477 & 1.654088 & 0.914579 & 0.536688 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 2 & 0.883633 & 214 & 477 & 1.255765 & 0.883633 & 0.448637 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 3 & 0.864953 & 187 & 477 & 1.020964 & 0.864953 & 0.392034 & Llama3.1-8B-AA \\
Mistral-7B-AA 1 & 0.897552 & 267 & 477 & 1.834382 & 0.897552 & 0.559748 & Mistral-7B-AA \\
Mistral-7B-AA 2 & 0.877562 & 237 & 477 & 1.557652 & 0.877562 & 0.496855 & Mistral-7B-AA \\
Mistral-7B-AA 3 & 0.865671 & 212 & 477 & 1.329140 & 0.865671 & 0.444444 & Mistral-7B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/synthpai/utility_model_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_model & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-3.5-AA 1 & 0.956918 & 261 & 477 & 1.817610 & 0.956918 & 0.547170 & GPT-3.5-AA \\
GPT-3.5-AA 2 & 0.946751 & 243 & 477 & 1.637317 & 0.946751 & 0.509434 & GPT-3.5-AA \\
GPT-3.5-AA 3 & 0.939832 & 224 & 477 & 1.457023 & 0.939832 & 0.469602 & GPT-3.5-AA \\
GPT-4-AA 1 & 0.937631 & 182 & 477 & 0.958071 & 0.937631 & 0.381551 & GPT-4-AA \\
GPT-4-AA 2 & 0.916247 & 140 & 477 & 0.624738 & 0.916247 & 0.293501 & GPT-4-AA \\
GPT-4-AA 3 & 0.898532 & 125 & 477 & 0.511530 & 0.898532 & 0.262055 & GPT-4-AA \\
Llama3.1-70B-AA 1 & 0.935639 & 187 & 477 & 1.037736 & 0.935639 & 0.392034 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 2 & 0.918029 & 162 & 477 & 0.756813 & 0.918029 & 0.339623 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 3 & 0.899371 & 149 & 477 & 0.637317 & 0.899371 & 0.312369 & Llama3.1-70B-AA \\
Llama3.1-8B-AA 1 & 0.925052 & 256 & 477 & 1.654088 & 0.925052 & 0.536688 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 2 & 0.903983 & 214 & 477 & 1.255765 & 0.903983 & 0.448637 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 3 & 0.892243 & 187 & 477 & 1.020964 & 0.892243 & 0.392034 & Llama3.1-8B-AA \\
Mistral-7B-AA 1 & 0.946646 & 267 & 477 & 1.834382 & 0.946646 & 0.559748 & Mistral-7B-AA \\
Mistral-7B-AA 2 & 0.938470 & 237 & 477 & 1.557652 & 0.938470 & 0.496855 & Mistral-7B-AA \\
Mistral-7B-AA 3 & 0.929665 & 212 & 477 & 1.329140 & 0.929665 & 0.444444 & Mistral-7B-AA \\
\bottomrule
\end{tabular}


==> figures/plots/synthpai/utility_rouge_correct.tex <==
\begin{tabular}{lrrrrrrl}
\toprule
full_anon_setting & utility_rouge & \multicolumn{2}{r}{first_correct} & certainty & utility & correctness & hue \\
 & mean & sum & count & mean &  &  &  \\
\midrule
GPT-3.5-AA 1 & 0.889544 & 261 & 477 & 1.817610 & 0.889544 & 0.547170 & GPT-3.5-AA \\
GPT-3.5-AA 2 & 0.846925 & 243 & 477 & 1.637317 & 0.846925 & 0.509434 & GPT-3.5-AA \\
GPT-3.5-AA 3 & 0.804962 & 224 & 477 & 1.457023 & 0.804962 & 0.469602 & GPT-3.5-AA \\
GPT-4-AA 1 & 0.875106 & 182 & 477 & 0.958071 & 0.875106 & 0.381551 & GPT-4-AA \\
GPT-4-AA 2 & 0.765517 & 140 & 477 & 0.624738 & 0.765517 & 0.293501 & GPT-4-AA \\
GPT-4-AA 3 & 0.690859 & 125 & 477 & 0.511530 & 0.690859 & 0.262055 & GPT-4-AA \\
Llama3.1-70B-AA 1 & 0.897865 & 187 & 477 & 1.037736 & 0.897865 & 0.392034 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 2 & 0.825174 & 162 & 477 & 0.756813 & 0.825174 & 0.339623 & Llama3.1-70B-AA \\
Llama3.1-70B-AA 3 & 0.774141 & 149 & 477 & 0.637317 & 0.774141 & 0.312369 & Llama3.1-70B-AA \\
Llama3.1-8B-AA 1 & 0.893632 & 256 & 477 & 1.654088 & 0.893632 & 0.536688 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 2 & 0.842932 & 214 & 477 & 1.255765 & 0.842932 & 0.448637 & Llama3.1-8B-AA \\
Llama3.1-8B-AA 3 & 0.810373 & 187 & 477 & 1.020964 & 0.810373 & 0.392034 & Llama3.1-8B-AA \\
Mistral-7B-AA 1 & 0.799365 & 267 & 477 & 1.834382 & 0.799365 & 0.559748 & Mistral-7B-AA \\
Mistral-7B-AA 2 & 0.755746 & 237 & 477 & 1.557652 & 0.755746 & 0.496855 & Mistral-7B-AA \\
Mistral-7B-AA 3 & 0.737682 & 212 & 477 & 1.329140 & 0.737682 & 0.444444 & Mistral-7B-AA \\
\bottomrule
\end{tabular}

